Semi-Centennial REDUCE

We present a version of the REDUCE computer algebra system as it was in the early 1970s. We show how this historical version of REDUCE may be built and run in very modest present-day environments and outline some of its capabilities.

==> IfExistsUseBBL.tex <==
% If this file exists, then the .bbl file is used instead of calling bibtex.
% It cannot be empty.   To force bibtex to run, rename this file to something else.
